Artificial Replay: A Meta-Algorithm for Harnessing Historical Data in Bandits

Most real-world deployments of bandit algorithms exist somewhere in between the offline and online set-up, where some historical data is available upfront and additional data is collected dynamically online. How best to incorporate historical data to "warm start" bandit algorithms is an open question: naively initializing reward estimates using all historical samples can suffer from spurious data and imbalanced data coverage, leading to data inefficiency (amount of historical data used) - particularly for continuous action spaces. To address these challenges, we propose ArtificialReplay, a meta-algorithm for incorporating historical data into any arbitrary base bandit algorithm. We show that ArtificialReplay uses only a fraction of the historical data compared to a full warm-start approach, while still achieving identical regret for base algorithms that satisfy independence of irrelevant data (IIData), a novel and broadly applicable property that we introduce. We complement these theoretical results with experiments on K-armed bandits and continuous combinatorial bandits, on which we model green security domains using real poaching data. Our results show the practical benefits of ArtificialReplay for improving data efficiency, including for base algorithms that do not satisfy IIData.

==> parts/acknowledgments.tex <==
\subsubsection*{Acknowledgments}
Part of this work was done while Sid Banerjee, Sean Sinclair, and Christina Lee Yu were visiting the Simons Institute for the Theory of Computing for the semester on Data-Driven Decision Processes. This work was supported, in part, by the NSF under grants ECCS-1847393, DMS-1839346, CCF-1948256, and CNS-1955997, and the ARL under grant W911NF-17-1-0094.  Lily Xu acknowledges the support of a Google PhD Fellowship. 

==> parts/full_model.tex <==
\section{Full Preliminary Details}
\label{sec:app_preliminary}

 In this section we restate and give further assumptions for the general stochastic bandit model described in \cref{sec:preliminary}.

\begin{comment}

\subsection{$K$-Armed Bandit}

The finite-armed bandit model can be viewed in this framework by considering $\actionset = [K] = \{1, \ldots, K\}$.  This recovers the classical model from \cite{lai1985asymptotically,auer2002finite}.

\subsection{Combinatorial Multi-Armed Bandit for Continuous Resource Allocation (\CMABCRA)}

A central planner has access to a metric space~$\pointset$ of resources with metric~$d_\pointset$.  They are tasked with splitting a total amount of $\budget$ divisible budget across $N$~different resources within~$\pointset$.  For example, in a wildlife conservation domain, the space~$\pointset$ can be considered as the protected area of a park, and the allocation budget corresponds to divisible effort, or proportion of rangers allocated to patrol in the chosen area.  We denote the feasible space of allocations as~$\effortset$ and define the feasible action space as follows:
\begin{align}
    \actionset = \left\{ (\points, \effort) \in \pointset^N \times \effortset^N \bigm\vert \sum_{i=1}^N \efforti{i} \leq \budget, \quad d_\pointset(\pointi{i},\pointi{j}) \geq \epsilon \quad \forall i \neq j \right\} \ .
\end{align}
Note that we require the chosen action to satisfy the budgetary constraint (i.e. $\sum_i \efforti{i} \leq \budget$), and that the chosen resources are distinct (aka $\epsilon$-away from each other according to $d_\pointset$).


Further, let $\rewarddist : \pointset \times \effortset \rightarrow \Delta([0,1])$ be the \emph{unknown} reward distribution over the resource and allocation space. The goal of the algorithm is to pick an action $\action = (\points, \effort) \in \actionset$ in a way that maximizes $\sum_{i=1}^N \Exp{\rewarddist(\pointi{i}, \efforti{i})}$, the expected total mean reward accumulated from the resources subject to the budget constraints. Denoting $\Exp{\rewarddist(\point, \effortgeneric)}$ as $\reward(\point, \effortgeneric)$, the optimization problem is formulated below:
\begin{align}
    \max_{\points, \effort} & \, \sum_{i=1}^N \reward(\pointi{i}, \efforti{i}) \label{eq:cmab_opt_appendix} \\
    \text{s.t. } & \sum_i \efforti{i} \leq B \nonumber\\
    & d_\pointset(\pointi{i}, \pointi{j}) \geq \epsilon \quad \forall i \neq j \ . \nonumber
\end{align}

Lastly, we consider the historical data $\history$ to also be decomposed, in that each element is a particular $(\point, \effortgeneric, \obsrewardt{})$ pair with $\obsrewardt{} \sim \rewarddist(\point, \effortgeneric)$.

\subsubsection{Assumptions}

We make two assumptions on the underlying problem.  The first is a standard nonparametric assumption, highlighting that the resource space~$\pointset$ is a metric space and that the true underlying reward function~$\reward$ is Lipschitz with respect to~$d_\pointset$.  This assumption is common in the continuous bandit literature; see \cite{kleinberg2019bandits} for more discussion.

\begin{assumption}
$\pointset$ is a compact metric space endowed with a metric~$d_\pointset$ with diameter~$\dmax$, and $\effortset$~is a discrete space, both known to the decision maker.  We assume that the mean reward function $\reward(\point, \effortgeneric)$ is Lipschitz with respect to the metric~$d_\pointset$ over $\point$ with known Lipschitz constant~$L$.
\end{assumption}

The next assumption assumes access to an oracle for solving optimization problems of the form of \cref{eq:cmab_opt} for arbitrary choice of reward functions $r(\point, \effortgeneric)$.  We can relax this assumption to instead assume that there exists a randomized approximation oracle by appropriately shifting the regret benchmark.  However, in \cref{sec:experiments} we run experiments with exact solution oracles and omit this discussion from this work.

\begin{assumption}
The optimization problem formulated in \cref{eq:cmab_opt} can be solved for arbitrary reward functions $\reward(\point, \effortgeneric)$.
\end{assumption}


\subsubsection{Mapping to Green Security Domains} 
The \CMABCRA model can be used to specify green security domains from \cite{xu2021dual}.  $\pointset$~is used to represent the ``protected region'', or geographic region of the park, and $\effortset$~is the discrete set of potential patrol efforts to allocate, such as the number of ranger hours per week, with the total budget~$B$ being $40$~hours.  This formulation generalizes \cite{xu2021dual} to a more realistic continuous space model of the landscape, instead of the artificial fixed discretization that was considered in prior work consisting of $1 \times 1$ sq.~km regions on park).

\end{comment}

\subsection{Historical Dataset}
\label{sec:app_preliminary_historical}

We assume that the algorithm designer has access to a historical dataset $\history = \{\actionhistt{j}, \rewardhistt{j}\}_{j\in[H]}$ containing $H$ historical points with actions~$\actionhistt{j}$ and rewards~$\rewardhistt{j}$ sampled according to $\rewarddist(\actionhistt{j})$.

We briefly discuss the required assumptions on how the dataset is chosen in order for $\Full$ and $\ArtReplay$ to be a reasonable algorithm for incorporating historical data in the first place.  We first give two examples:
\begin{itemize}
\item The historical dataset is sampled according to a fixed, non-adaptive policy.  In this case we have that $H_a$, the number of samples for each arm is selected apriori, and each sample $\actionhistt{j}$ has rewards~$\rewardhistt{j}$ sampled according to $\rewarddist(\actionhistt{j})$
\item The historical dataset is sampled using an \iidata algorithm.  Then the number of samples from each action $H_a$ is a random variable, but each observed reward has the correct marginal distribution by being sampled according to $\rewarddist(\actionhistt{j})$.
\end{itemize}

However, there are many scenarios on how the historical dataset is generated that could lead to \Full nor \ArtReplay to be the right algorithm in the first place.  For a simple example, suppose that the samples for each arm $a$ were sorted in decreasing order.  In this case, \ArtReplay will learn biased estimates of the underlying mean reward by not using the entire historical dataset.  Similarly, suppose that the historical dataset was sampled according to an algorithm that ``ignored'' samples smaller than a certain threshold value.  Both \Full and \ArtReplay would again learn biased estimates of the mean reward for the actions from this historical data.

We leave the interesting question of when \Full and \ArtReplay are the optimal heuristics for incorporating dataset due to tampering of the historical data for future work.

==> parts/introduction_old.tex <==
% \srscomment{SEAN DO THIS}
% $\action$, $\actiongeneric$, $\actiont{}, \actionhist, \actionhistt{j}$

% $\obsreward, \rewarddist, \rewardhist, \rewardhistt{j}$

\section{Introduction}

Multi-armed bandits and their variants are robust models for many real-world problems. Resulting algorithms have been applied to wireless networks~\citep{zuo2021combinatorial}, COVID testing regulations~\citep{bastani2021efficient}, and conservation efforts to protect wildlife from poaching~\citep{xu2021dual}.  Typically, algorithm designers assume no prior knowledge of the mean rewards of each action, designing algorithms to address the \emph{exploration--exploitation trade-off} by exploring actions for additional informational value. However, in many applications we have access to \emph{prior data} about the actions. For example, in the context of wildlife conservation, there is rich information on historical patrols that should be incorporated to learn poaching risk before deploying any bandit algorithm, and subsequently we incur significant losses by ignoring such prior data.  %poaching patterns from a park can be incorporated into another park's bandit algorithm.

While we commonly have access to a \emph{generous amount of historical data}, there is no consensus on how to optimally incorporate this data into online learning algorithms. One challenge is that we have no control over the policy under which the historical data was collected, so there may be \emph{imbalanced data coverage}, where samples are highly non-uniformly distributed. Furthermore, the historical policy could be inefficient and suboptimal, leading to \emph{spurious data} with excessive data collected on poorly performing actions. Both of these issues could result in a scenario where the usefulness of the dataset is only moderate, despite the size of the dataset being extremely large.
As a result, naively processing the entire historical dataset to initialize reward estimates could involve unnecessary and onerous computation and storage burdens, whereas a wisely chosen subset of the data could contain equally informative value. For example, only a bounded number of samples are needed to rule out a sub-optimal action, whereas the dataset may contain unnecessarily excessive data on such sub-optimal actions. Indeed, \cite{martin2017timing} notes that for conservation decision making, more information does not always translate into better actions;  time is the resource which matters most.


% \lily{ \cite{martin2017timing} Add discussion to this paragraph?}
% reminding everyone that more information does not always translate into more efficacious action may help strike a better balance between action and research. When it comes to species conservation, time is the resource that matters most

%We define historical data as any observations from actions that are collected independently of the online learning algorithm. 
Hypothetically, if we could \emph{choose} which samples to include in the historical dataset, a natural approach would be to use a regret-optimal bandit algorithm to guide the sampling of the historical data.  Based on this philosophy, we propose \ArtReplay, a meta-algorithm that modifies any arbitrary base bandit algorithm to harness historical data.  Our approach reduces computation and storage costs by only using historical data on an \emph{as needed} basis. 
At a high level, we artificially simulate online actions using historical data as a replay buffer.  Every time the base algorithm picks an action, we first check the historical data for any unused samples from the chosen action. If an unused sample exists, update the estimates and continue without advancing to the next timestep.  Otherwise, sample from the environment, use the observed data to update the estimates, and continue to the next timestep. In contrast, a ``full warm start'' modification of the same base algorithm would first preprocess the entire historical dataset and initialize the estimates accordingly before beginning any online actions. 

We show an \emph{exact coupling} (i.e., identical distribution over sample paths) between our \ArtReplay approach and the ``full warm start'' approach with the same base algorithm, as long as the base algorithm satisfies a novel \emph{independence of irrelevant data} (\iidata) assumption.  This coupling highlights how the \ArtReplay framework achieves regret \emph{identical} to the ``full warm start'' approach while also guaranteeing significantly better time and storage complexity.  We provide examples of regret optimal algorithms which satisfy the \iidata assumption, and we conclude with an empirical analysis, applied to green security domains with real-life poaching data from Uganda.


\paragraph{Contributions}  We address the real-world characteristics of harnessing historical data in online bandit algorithms.  Concretely, we propose \ArtReplay, a meta-algorithm that modifies {\em any arbitrary base bandit algorithm} to incorporate historical data.  We show that a sub-class of algorithms satisfying a novel \emph{independence of irrelevant data} (\iidata) property has an explicit sample-path coupling between the regret of the \ArtReplay approach and full warm start.  To highlight the breadth of algorithms satisfying the \iidata property, we give examples of regret-optimal \iidata polices for the $K$-armed and continuous combinatorial bandits. We complement these examples by showing that \ArtReplay can lead to arbitrary better storage and computational complexity requirements.  Finally, we perform a case-study of combinatorial bandit algorithms for continuous resource allocation in the context of green security domains.  We propose several algorithms to tackle this problem, including a novel adaptive discretization technique.  Across the experiments, we observe concrete gains in storage and runtime using real-world poaching data from the \ArtReplay framework over a wide range of base algorithms. 
%Note that all proofs are deferred to \cref{app:proofs}.
% removed this comment as that should probably be obvious for short conference papers

